An Empirical Study on the Usage of Automated Machine Learning Tools

The popularity of automated machine learning (AutoML) tools in different domains has increased over the past few years. Machine learning (ML) practitioners use AutoML tools to automate and optimize the process of feature engineering, model training, and hyperparameter optimization and so on. Recent work performed qualitative studies on practitioners' experiences of using AutoML tools and compared different AutoML tools based on their performance and provided features, but none of the existing work studied the practices of using AutoML tools in real-world projects at a large scale. Therefore, we conducted an empirical study to understand how ML practitioners use AutoML tools in their projects. To this end, we examined the top 10 most used AutoML tools and their respective usages in a large number of open-source project repositories hosted on GitHub. The results of our study show 1) which AutoML tools are mostly used by ML practitioners and 2) the characteristics of the repositories that use these AutoML tools. Also, we identified the purpose of using AutoML tools (e.g. model parameter sampling, search space management, model evaluation/error-analysis, Data/ feature transformation, and data labeling) and the stages of the ML pipeline (e.g. feature engineering) where AutoML tools are used. Finally, we report how often AutoML tools are used together in the same source code files. We hope our results can help ML practitioners learn about different AutoML tools and their usages, so that they can pick the right tool for their purposes. Besides, AutoML tool developers can benefit from our findings to gain insight into the usages of their tools and improve their tools to better fit the users' usages and needs.

==> tables/tbl_tools_correlation_appriori.tex <==

% https://sqa.stackexchange.com/questions/7391/mutation-testing-fault-injection-robustness-testing-fuzz-testing

\begin{table}[!h]

%\large
\caption{\textbf{Apriori details}:}
\label{tab:apriori}
%\scalebox{0.55}{
%\resizebox{.99\textwidth}{!}{

\begin{adjustbox}{width=.5\textwidth}
%\scalebox{0.75}{
 % \centering
 %\resizebox*{!}{5cm}{%
%\resizebox*{.5\textwidth}{!}{% <------ Don't forget this %

 \begin{tabular}{c|l |c c c}\toprule
  
  \rowcolor{gray!15}
  \textbf{antecedents}&\textbf{consequents}&\textbf{support}&\textbf{confidence}&\textbf{lift}\\ 
 \midrule
 %\midrule
 
     \multirow{2}{*}{\textbf{Optuna}} 
    % &neptune-contrib&0.001790&0.010945&4.47419\\ 
     &tpot&0.001700&0.010398&0.120477\\ 
     &hyperopt&0.003043&0.018606&0.118327\\ \hline
     
     \multirow{4}{*}{\textbf{hyperopt}} 
     &hpsklearn&0.001193&0.007589&1.382503\\ 
     &tpot&0.002834&0.018023&0.208833\\ 
     &skopt&0.001581&0.010055&0.120076\\
     &optuna&0.003043&0.019351&0.118327\\\hline
     
     \multirow{3}{*}{\textbf{skopt}} 
    % &ray&0.000984&0.011756&1.743733\\ 
     &hyperopt&0.001581&0.018881&0.120076\\ 
     &bayes\_opt&0.000686&0.008194&0.088118\\
     &optuna&0.000507&0.006056&0.037033\\\hline
     
     \multirow{3}{*}{\textbf{featuretools}} 
     &evalml&0.000507&0.016144&2.254895\\ 
     &tpot&0.000388&0.012346&0.143049\\ 
     &optuna&0.000328&0.010446&0.063877\\ \hline
     
     \multirow{3}{*}{\textbf{tpot}} 
     &hpsklearn&0.000537&0.006222&1.133504\\ 
     &hyperopt&0.002834&0.032838&0.208833\\ 
     &optuna&0.001700&0.019703&0.120477\\\hline

     \multirow{3}{*}{\textbf{bayes\_opt}} 
     &skopt&0.000686&0.007379&0.088118\\ 
     &hyperopt&0.000626&0.006737&0.042846\\ \hline 
 
     \multirow{1}{*}{\textbf{autokeras}} 
     &kerastuner&0.001372&0.036537&1.164215\\
     \hline
     

     
     \multirow{1}{*}{\textbf{auto-sklearn}} 
     &tpot&0.000418&0.014374&0.166547\\
     \hline
 
     \multirow{1}{*}{\textbf{Ax}} 
     &-&-&-&-\\ \hline

     \multirow{1}{*}{\textbf{snorkel}} 
     &-&-&-&-\\ 
     

     
 
\bottomrule
 \end{tabular}
 %}
%  
 \end{adjustbox}
%}
\vspace{10pt}
\end{table}
